GS-Playground: A High-Throughput Photorealistic Simulator for Vision-Informed Robot Learning

Embodied AI research is undergoing a shift toward vision-centric perceptual paradigms. While massively parallel simulators have catalyzed breakthroughs in proprioception-based locomotion, their potential remains largely untapped for vision-informed tasks due to the prohibitive computational overhead of large-scale photorealistic rendering. Furthermore, the creation of simulation-ready 3D assets heavily relies on labor-intensive manual modeling, while the significant sim-to-real physical gap hinders the transfer of contact-rich manipulation policies. To address these bottlenecks, we propose GS-Playground, a multi-modal simulation framework designed to accelerate end-to-end perceptual learning. We develop a novel high-performance parallel physics engine, specifically designed to integrate with a batch 3D Gaussian Splatting (3DGS) rendering pipeline to ensure high-fidelity synchronization. Our system achieves a breakthrough throughput of 10^4 FPS at 640x480 resolution, significantly lowering the barrier for large-scale visual RL. Additionally, we introduce an automated Real2Sim workflow that reconstructs photorealistic, physically consistent, and memory-efficient environments, streamlining the generation of complex simulation-ready scenes. Extensive experiments on locomotion, navigation, and manipulation demonstrate that GS-Playground effectively bridges the perceptual and physical gaps across diverse embodied tasks. Project homepage: https://gsplayground.github.io.

==> Assets/Figures/grasp_balance_force.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{Assets/Figures/images/grasp_balance_force_top.pdf}
    \caption{\textbf{Vertical force balance in a Panda grasp.}
    The plot compares the vertical contact support force $F_z$ with the theoretical object weight $mg$ during lift, settling, and hold. MuJoCo Euler exhibits large oscillatory contact forces, while \method and MuJoCo FastImplicit remain close to the force-balance target.}
    \label{fig:grasp_force_balance}
\end{figure}


==> Assets/Figures/rolling_ball_scene.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Assets/Figures/images/rolling_ball_scene.jpg}
    \caption{\textbf{Ball falling Scene:} A ball falls onto the inclined plane.}
    \label{fig:ball_falling_scene}
\end{figure}


==> Assets/Figures/rolling_friction_normal_force_comparison.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{Assets/Figures/images/rolling_friction_normal_force_comparison.pdf}
    \caption{\textbf{Rolling friction normal force.}
    This diagram compares the normal force acting on the small ball after it contacts the inclined plane.}
    \label{fig:rolling_friction_comparison}
\end{figure}


==> Assets/Figures/shaking_scene.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.5\linewidth]{Assets/Figures/images/shaking_scene.pdf}
\caption{\textbf{Shaking Test Scene}: A Franka Panda robot grasps various objects (a cube, a ball, and a bottle) while being subjected to random shaking motions. This setup is used to evaluate the grasping robustness of different simulation methods under dynamic perturbations.}
\vspace{-4mm}
\label{fig:shaking_scene}
\end{figure}


==> Assets/Tables/critical_friction_hold_test.tex <==
\begin{table}[t]
    \centering
    \caption{\small \textbf{Critical-friction hold test}. Each trial starts from the initialized Panda grasp hold state and runs for 5\,s with friction coefficient $\mu=\alpha\mu_{\mathrm{crit}}$. Here $\mu_{\mathrm{crit}}=mg/N=0.0902$, with $N\approx6.962$\,N and $mg=0.6278$\,N. Numeric entries report the first drop time in seconds; $\checkmark$ indicates the object remained held for the full trial. $\dagger$ marks an outcome that violates the theoretical hold/drop expectation.}
    \setlength{\tabcolsep}{3pt}
    \scalebox{0.95}{
        \begin{tabular}{lccccc}
            \toprule
            \textbf{Engine} & \textbf{0.90x} & \textbf{0.98x} & \textbf{1.00x} & \textbf{1.02x} & \textbf{1.10x} \\
            \midrule
            Theory & Drop & Drop & Hold & Hold & Hold \\
            \midrule
            \method & 0.10 & 0.25 & \textbf{$\checkmark$} & \textbf{$\checkmark$} & \textbf{$\checkmark$} \\
            MuJoCo Euler & 0.07 & 0.08 & 0.08$^\dagger$ & 0.08$^\dagger$ & 0.07$^\dagger$ \\
            MuJoCo FastImplicit & 0.10 & 0.21 & 1.23$^\dagger$ & 2.00$^\dagger$ & 2.70$^\dagger$ \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:critical_friction_hold}
\end{table}


==> Assets/Tables/franka_shaking.tex <==

\begin{table}[t]
    \centering
    \caption{\small \textbf{Grasping robustness under external disturbances}. Success rates for a Franka Panda holding various geometries (cube, ball, bottle) under random shaking. A trial is successful if the object is retained for the entire evaluation horizon. 
    }
    \scalebox{1}{
        \begin{tabular}{lcc}
            \toprule
            \textbf{Engine} & \textbf{dt=0.002s (success)} & \textbf{dt=0.01s (success)} \\
            \midrule
            MuJoCo (Euler) & 0/90 & 0/90 \\
            MuJoCo (Implicit) & 0/90 & 0/90 \\
            MuJoCo (Implicit+Noslip) & 4/90 & 0/90 \\
            MJWarp & 0/90 & 10/90 \\
            IsaacSim & 60/90 & 60/90 \\
            Genesis & 60/90 & 60/90 \\
            Ours (CPU) & \textbf{90/90} & \textbf{90/90} \\
            Ours (GPU) & \textbf{90/90} & \textbf{74/90} \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:franka_shaking}
\end{table}


==> Assets/Tables/grasp_balance_force_error.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Hold-stage vertical force-balance error.}
    Mean absolute error between the measured vertical support force $F_z$ and the object weight $mg$ for the hold phase in Fig.~\ref{fig:grasp_force_balance}.}
    \label{tab:grasp_force_balance_error}
    \setlength{\tabcolsep}{5pt}
    \scalebox{0.95}{
        \begin{tabular}{lc}
            \toprule
            \textbf{Engine} & \textbf{Mean $\lvert F_z - mg \rvert$ (mN)} \\
            \midrule
            Ours & \textbf{0.039} \\
            MuJoCo FastImplicit & 0.039 \\
            MuJoCo Euler & 1740.233 \\
            \bottomrule
        \end{tabular}
    }
\end{table}

